MASAI: Modular Architecture for Software-engineering AI Agents

A common method to solve complex problems in software engineering, is to divide the problem into multiple sub-problems. Inspired by this, we propose a Modular Architecture for Software-engineering AI (MASAI) agents, where different LLM-powered sub-agents are instantiated with well-defined objectives and strategies tuned to achieve those objectives. Our modular architecture offers several advantages: (1) employing and tuning different problem-solving strategies across sub-agents, (2) enabling sub-agents to gather information from different sources scattered throughout a repository, and (3) avoiding unnecessarily long trajectories which inflate costs and add extraneous context. MASAI enabled us to achieve the highest performance (28.33% resolution rate) on the popular and highly challenging SWE-bench Lite dataset consisting of 300 GitHub issues from 11 Python repositories. We conduct a comprehensive evaluation of MASAI relative to other agentic methods and analyze the effects of our design decisions and their contribution to the success of MASAI.

==> Backup/1_intro_backup.tex <==
% \begin{figure}
% \includegraphics[width=\textwidth]{Images/agent.jpg}
% \caption{The GoalKeeper modular architecture of goal-oriented AI agents}
% \label{fig:overview}
% \end{figure}

Large language models have shown remarkable ability to reason~\citep{kojima2022large} and plan~\cite{huang2022language}.
Multi-step or iterative reasoning, structured as chains~\citep{wei2022chain} or trees~\citep{yao2024tree} of thought, further enhance their ability to solve complex problems requiring many inter-related steps of reasoning. When combined with environment actions~\citep{yao2023react,patil2023gorilla} and feedback from the environment~\citep{zhou2023language,shinn2024reflexion}, they enable autonomous agents capable of achieving specific goals~\citep{zhang2023igniting}.

As the complexity of tasks increases, it becomes increasingly difficult to solve them without identifying the intermediate subgoals necessary to achieve the final outcome. 

In this paper, we propose a flexible agent architecture in which a high-level reasoning component, called GoalKeeper, modularizes a goal into subgoals and monitors the progress on those subgoals (Fig. 1). It can respond to the outcomes of subgoals and re-evaluate the plan. The subgoals are delegated to sub-agents. The GoalKeeper can pass relevant information across sub-agents. The modularity of our architecture allows the sub-agents to use any strategy, e.g.,~\citep{wei2022chain,yao2024tree,yao2023react,shinn2024reflexion,zhou2023language,lewis2020retrieval}, that is effective for the subgoal. To avoid interference between different sub-agents, they are not allowed to directly affect the environment. Rather, they work on local copies of the environment \aksays{Will this be perceived as too expensive?} and it is the GoalKeeper that decides whether any of the updates to the local environment should also be applied to the global environment. Thus, the sub-agents can experiment with the local environment without the fear of catastrophic side-effects. The success of the task is determined by whether the global environment reaches the goal state.

\aksays{We need a concrete example from SWEBench where both SWE-Agent and OpenDevin fail and we succeed and the success can be attribued to modularity or our design philosophy in general. In particular, we want to show that disparate sources of information are essential to solve the issue which can be visualized by giving partial directory listings and putting different symbols/colors against relevant documents (e.g., a README, a test file, a new test file that is created, a trail of reasoning during localization, etc.)}

Why modularity
\begin{itemize}
\item Ability to perform specialized reasoning in different phases of the task, e.g., use React to gather information and understand the environment, and use CoT when sufficient information is available
\item Gather information from multiple sources independently, e.g., a README, a test, imported files, etc. - should not spring into action without the right context
\item Control length, complexity and noise in trajectories to avoid distracting the LM
\item Control unintended side-effects and provide appropriate pre-requisites for different sub-tasks, e.g., restore the repo after print statements are added for debugging purposes, ensure that the runtime environment is set up, etc.
\item Explore capability-cost tradeoff by enabling different models to be plugged in for different sub-tasks, e.g., SLMs are faster and cost-effective
\end{itemize}

As a demonstration of effectiveness of the GoalKeeper architecture, we experiment with a diverse set of software development tasks requiring repository-wide changes. [Details of datasets, baselines and results] SWEBench~\cite{jimenez2023swe}

Are we using existing tests and double validation and test anchors from alphacodium?

we perform eval in a setting faithful to the proposed SWEBench setting 

we provide both ACI and shell access (which is useful as discussed in the localization RQ)

Contributions
\begin{itemize}
\item We present a modular architecture, MASAI, comprising well-designed sub-agents that are effective at solving specific repository-wide sub-tasks.
\item We establish a new state-of-the-art (SOTA) on the challenging SWEBench-lite benchmark surpassing all the existing approaches, demonstrating the effectiveness of MASAI over the prevailing single agent architectures. \aksays{We have to make it clear that there are no multi-agent baselines to compare against.}
\item We conduct a thorough evaluation of effectiveness of both fine-grained components and high-level solution strategies across MASAI and recent SOTA approaches (SWE-Agent and OpenDevin), offering insights for future work.
\item We will release our data and evaluation scripts.
\end{itemize}

==> Backup/1_intro_backup_june_14.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{@{}c@{}c@{}c@{}}
    \includegraphics[width=0.32\linewidth]{Images/resolution_v_cost.png} &
    \includegraphics[width=0.32\linewidth]{Images/interactions_v_tokens.png} &        \includegraphics[width=0.32\linewidth]{Images/interactions_v_cost.png}\\
    (a) Avg. cost vs. resolution rate &
    (b) \#interactions vs. token cost &
    (c) \#interactions vs. dollar cost
    \end{tabular}
    \caption{Comparison of \sysname with existing methods.
    \textbf{Legend:}
    \emph{Resolution rate} refers to the percentage of issues in \datasetsmall that are resolved. \emph{Number of interactions} refers to the number of interactions between the LLM and the agent environment. In plots (b) and (c), each run of an agent over an issue is mapped to a point. For each agent, the runs are sorted in the increasing order of \#interactions. All prior works from plot (a) whose logs were available with the relevant information are included in plots (b) and (c). Note that the Y-axes for (b) and (c) are in \emph{log-scale}.
    \textbf{Results:} 
    Plot (a) shows that \sysname achieves the highest resolution rate at a very low (average) cost. Plot (b) shows that \sysname facilitates more number of interactions between the LLM and the environment, yet it consumes much lower tokens because of the modular architecture where each sub-agent is focused and frugal. Plot (c) similarly shows that modularity helps \sysname incur lower cost.
    \aksays{Increase font sizes within figures and minimize margins between axis-labels and plots.}
    }
    \label{fig:cost_scatter}
\end{figure}

Software engineering is a challenging activity which requires exercising various skills such as coding, reasoning, testing and debugging. The ever growing demand for software calls for better support to software engineers. The recent advances in AI offer much promise in this direction.

Large language models (LLMs) have shown remarkable ability to code~(\cite{chen2021evaluating,roziere2023code,codegemma}, \emph{inter alia}), reason~\citep{kojima2022large} and plan~\citep{huang2022language}. Iterative reasoning, structured as chains~\citep{wei2022chain} or trees~\citep{yao2024tree} of thought, further enhance their ability to solve complex problems requiring many inter-related steps of reasoning. When combined with tools or environment actions~\citep{yao2023react,patil2023gorilla,schick2024toolformer} and feedback from the environment~\citep{zhou2023language,shinn2024reflexion}, they enable autonomous agents capable of achieving specific goals~\citep{zhang2023igniting}.

As the problem complexity increases, it becomes difficult to devise a single, over-arching strategy that works across the board. Indeed, when faced with a complex coding problem, software engineers break it down into sub-problems and use different strategies to deal with them separately. Inspired by this, we propose a Modular Architecture of Software-engineering AI (\sysname) agents, where different sub-agents are instantiated with well-defined objectives and strategies tuned to achieve those objectives. The sub-agents are powered by LLMs.

Our modular architecture offers several advantages: (1)~employing and tuning different problem-solving strategies across sub-agents (e.g., ReAct or CoT), (2)~enabling sub-agents to gather information from different sources scattered throughout a repository (e.g., from a README, a test file or a source-code file), and (3)~avoiding unnecessarily long trajectories which are difficult to reason about and inflate inference costs.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\linewidth]{Images/interactions_vs_cost.png}
%         \includegraphics[width=0.45\linewidth]{Images/interactions_vs_tokens.png}
%     \caption{Cost vs Number of Interactions}
%     \label{fig:interaction_vs_cost}
% \end{figure}


We evaluate \sysname on the popular \datasetsmall dataset~\citep{jimenez2023swe} of 300 GitHub issues from 11 Python repositories. Due to its practical relevance and challenging nature, \datasetsmall has attracted significant efforts from academia, industry and start-ups.
As shown in Figure~\ref{fig:cost_scatter}(a), with the highest resolution rate of \sota, \sysname achieves state-of-the-art results on \datasetsmall. A concurrent work, \coder~\citep{chen2024coder}, also achieves the same resolution rate, but at a much higher cost of \codercost per issue, compared to our cost of \sotacost.
% \footnote{\todo{We consider all approaches published up to 2 weeks before the writing of this paper.}}
% Further, \sysname does so with the lowest average cost of \sotacost per issue.
This is possible because each sub-agent in \sysname is focused on a specific sub-problem and passes only the information necessary for the sub-problem to the LLM in a frugal manner. This is illustrated in plots (b) and (c) in Figure~\ref{fig:cost_scatter}.
\sysname sub-agents collectively facilitate more interactions between the LLM and the environment, while consuming significantly smaller number of tokens, resulting in lower costs.
Another recent work, Moatless~\citep{moatless}, has cost (\moatlesscost) lower than ours but also a lower resolution rate (\moatlessRR). We believe that both, the success at software engineering tasks and the cost are important factors to make these technologies effective and affordable.

% \aksays{We need a concrete example from SWEBench where both SWE-Agent and OpenDevin fail and we succeed and the success can be attributed to modularity or our design philosophy in general. In particular, we want to show that disparate sources of information are essential to solve the issue which can be visualized by giving partial directory listings and putting different symbols/colors against relevant documents (e.g., a README, a test file, a new test file that is created, a trail of reasoning during localization, etc.)}

The field of AI agents, and specifically software-engineering AI agents, is nascent.
AI agents for software engineering would likely encounter many common sub-problems, spanning from the ability to autonomously understand the testing infrastructure and code organization of a repository, writing new tests, to localizing a bug, editing large files without introducing syntactic or semantic errors, and finally synthesizing fixes or writing new code.
We believe that it is crucial to understand how different strategies perform on these sub-problems.
We therefore conduct a thorough investigation into the performance of \sysname and all the existing methods on \datasetsmall, and present the impact of key design decisions on the success of AI agents.

% \aksays{Note some of the key observations such as MASAI through ReAct achieves best localization, etc. We hope these observations would be useful in future research.}

% \aksays{Contributions}

In summary, we make the following contributions:
\begin{itemize}[leftmargin=10pt]
\item Propose a modular architecture, \sysname, that allows optimized design of sub-agents separately while combining them towards solving larger, end-to-end software engineering tasks autonomously.
\item Demonstrate the effectiveness of \sysname by achieving the highest resolution rate at a very low cost (an order of magnitude lower than the next equally successful method).
\item Conduct a thorough investigation into key design decisions of \sysname and the existing methods which can help inform future research and development in this rapidly evolving space.
\item Contribute our results to the \datasetsmall leaderboard~\citep{swebench_leaderboard} for validation.
\end{itemize}
